Synthetic CT Generation from MRI Using Improved DualGAN

Synthetic CT image generation from MRI scan is necessary to create radiotherapy plans without the need of co-registered MRI and CT scans. The chosen baseline adversarial model with cycle consistency permits unpaired image-to-image translation. Perceptual loss function term and coordinate convolutional layer were added to improve the quality of translated images. The proposed architecture was tested on paired MRI-CT dataset, where the synthetic CTs were compared to corresponding original CT images. The MAE between the synthetic CT images and the real CT scans is 61 HU computed inside of the true CTs body shape.

==> chapters/related_works.tex <==
%\section{Related Works}

%\begin{itemize}
   %\item 3 types of image-to-image translation    
   %\item Convolutional NN \& GAN and application to image translation (As mentioned before, it's applied)
   %\item GANs and paired image-to-image translation (MR-to-CT)
   %\item GANs and unpaired image-to-image translation (MR-to-CT)
%\end{itemize}
